Semi-Truths: A Large-Scale Dataset of AI-Augmented Images for Evaluating Robustness of AI-Generated Image detectors

Text-to-image diffusion models have impactful applications in art, design, and entertainment, yet these technologies also pose significant risks by enabling the creation and dissemination of misinformation. Although recent advancements have produced AI-generated image detectors that claim robustness against various augmentations, their true effectiveness remains uncertain. Do these detectors reliably identify images with different levels of augmentation? Are they biased toward specific scenes or data distributions? To investigate, we introduce SEMI-TRUTHS, featuring 27,600 real images, 223,400 masks, and 1,472,700 AI-augmented images that feature targeted and localized perturbations produced using diverse augmentation techniques, diffusion models, and data distributions. Each augmented image is accompanied by metadata for standardized and targeted evaluation of detector robustness. Our findings suggest that state-of-the-art detectors exhibit varying sensitivities to the types and degrees of perturbations, data distributions, and augmentation methods used, offering new insights into their performance and limitations. The code for the augmentation and evaluation pipeline is available at https://github.com/J-Kruk/SemiTruths.

==> sec/algorithms/SA_metric.tex <==
\begin{algorithm}
\caption{Post-Edit Surface Area Change ($I_{1}$, $I_{2}$)}
\label{algo:post-sa}
\begin{algorithmic}[1]
\State 
% \State \textcolor{blue}{Initialize key parameters}
% \State \textbf{Input:} $I_{1}$ (original image), $I_{2}$ (edited image)
% \State \textbf{Threshold:} $T \gets 0.1$
% \State \textbf{Kernel:} $K \gets \text{white\_pixels}(11,11)$
% \State \textcolor{blue}{\# Calculating mean squared error between the Real and Edited RGB images}
% \State $mse_{rgb} \gets (I_{1}[:,:,0] - I_{2}[:,:,0])^{2} + (I_{1}[:,:,1] - I_{2}[:,:,1])^{2} + (I_{1}[:,:,2] - I_{2}[:,:,2])^{2}$
% \State \textcolor{blue}{\# Normalization to (0,1)}
% \State $mse_{rgb}^{norm} \gets \frac{mse_{rgb}}{(255 \times 255 \times 3)}$
% \State \textcolor{blue}{\# Thresholding to remove noise}
% \State $mse\_thresh \gets \text{Remove\_Noise}(mse_{rgb}^{norm}, T)$
% \State \textcolor{blue}{\# Generate binary mask}
% \State $binary\_mask \gets mse\_thresh > 0$
% \State \textcolor{blue}{\# Dilate mask}
% \State $dilated\_mask \gets \text{Dilate}(binary\_mask, K)$
% \State \textcolor{blue}{\# Find all connected components for the mask}
% \State $\#CC, CC\_img, Stats, CC\_centroids \gets \text{Get\_connected\_components}(dilated\_mask)$
% \State \textcolor{blue}{\# Merge neighbouring components}
% \State $merged\_components \gets \text{Merge}(CC\_img, CC\_centroids)$
% \State \textcolor{blue}{\# Remove extremely small components to get final post edit mask}
% \State $post\_edit\_mask \gets \text{Remove\_Small}(merged\_components, \text{min\_size}, \text{min\_connected})$
% \State \textcolor{blue}{\# Calculate post edit ratio}
% \State $post\_edit\_ratio \gets \frac{\text{num\_white\_pixels}(post\_edit\_mask)}{\text{total\_pixels}(post\_edit\_mask)}$
% \State \textcolor{blue}{\# Calculate the largest distance between the connected components}
% \State $max\_centroid\_dist \gets \max(\text{pdist}(CC\_centroids))$
% \State \textcolor{blue}{\# Get the ratio of the largest connected component}
% \State $largest\_CC\_ratio \gets \frac{\max(\text{calc\_CC\_size}(Stats))}{\text{total\_pixels}(post\_edit\_mask)}$
% \State \textcolor{blue}{\# Categorize as localized or diffused change}
% \If {$largest\_CC\_ratio \geq 0.2$}
%     \State change $\gets$ \text{Diffused}
% \Else
%     \If {$\#CC > \text{mean}(\#CC)$ \And $max\_centroid\_dist > \text{dist\_thresh}$}
%         \State change $\gets$ \text{Diffused}
%     \Else
%         \State change $\gets$ \text{Localized}
%     \EndIf
% \EndIf
\end{algorithmic}
\end{algorithm}

